Improving Neural Networks for Time Series Forecasting using Data Augmentation and AutoML

Statistical methods such as the Box-Jenkins method for time-series forecasting have been prominent since their development in 1970. Many researchers rely on such models as they can be efficiently estimated and also provide interpretability. However, advances in machine learning research indicate that neural networks can be powerful data modeling techniques, as they can give higher accuracy for a plethora of learning problems and datasets. In the past, they have been tried on time-series forecasting as well, but their overall results have not been significantly better than the statistical models especially for intermediate length times series data. Their modeling capacities are limited in cases where enough data may not be available to estimate the large number of parameters that these non-linear models require. This paper presents an easy to implement data augmentation method to significantly improve the performance of such networks. Our method, Augmented-Neural-Network, which involves using forecasts from statistical models, can help unlock the power of neural networks on intermediate length time-series and produces competitive results. It shows that data augmentation, when paired with Automated Machine Learning techniques such as Neural Architecture Search, can help to find the best neural architecture for a given time-series. Using the combination of these, demonstrates significant enhancement in the forecasting accuracy of three neural network-based models for a COVID-19 dataset, with a maximum improvement in forecasting accuracy by 21.41%, 24.29%, and 16.42%, respectively, over the neural networks that do not use augmented data.

==> tex/0-abs.tex <==
\begin{abstract}
The abstract should briefly summarize the contents of the paper in
15--250 words.

\keywords{First keyword  \and Second keyword \and Another keyword.}
\end{abstract}

==> tex/1-intro.tex <==
Producing accurate forecasts for the COVID-19 Pandemic has been challenging due to the length of the time-series data that are available.
Only now is a full year's worth of data available for the United States (from January 22, 2020 to January 21, 2021).
The shortness of the time-series data is particularly a problem for machine learning models that require extensive training sets
in order to optimize their large sets of model parameters.

This paper examines the COVID-19 modeling studies that have been conducted and applies common modeling techniques from three broad categories:
(1) epidemiological models,
(2) statistical models, and
(3) machine learning models.
The first category of models applies scientific knowledge developed from past epidemics and pandemics as well as analysis of how infections are transmitted, e.g., likelihood of a Susceptible and Infected individual having enough contact to transmit the infection \cite{he2020seir,ferguson2020report,branas2020flattening,healthcare2020covid}.
The second category of models represents a robust and relatively easy to apply set of models that should be used in modeling studies (at least as point of comparison).
The third category, that of machine learning, supports more intense pattern matching that has the potential to produce more accurate forecasts.
The disadvantages include the necessity for more data, tuning of hyper-parameters, architecture search and interpretability.

Modeling studies are important for several reasons.
Forecasting is important, so people and their governments know what to expect in the next few weeks.
In addition, modeling studies are important for analyzing the effectiveness of Non-Pharmaceutical Interventions (NPI).

The COVID-19 Pandemic is unique in the sense that the last pandemic with this (or more) significance was the 1918 H1N1 Influenza Pandemic\cite{johnson2002updating,morens20101918}.
While the estimated global mortality of the pandemic was of the order of 50 million,\cite{johnson2002updating} believed that the real morbidity and mortality were substantially underestimated.  

Modeling and forecasting studies for COVID-19 are grouped into four major approaches:
a) SEIR/SIR models,
b) Agent-based models, 
c) Curve-fitting models, and
d) Predictive models.

\noindent \textbf{SEIR/SIR}\cite{lopez2020modified}
models are a common epidemiological modeling technique that predict the pandemic course through the system of equations that divide an estimated population into different compartments: susceptible, exposed, infected, and recovered.
A set of mathematical rules govern the equations as to how the assumptions about the disease process, Non-Pharmaceutical Interventions, social mixing and public vaccinations would affect the population.

\noindent \textbf{Agent-based}\cite{shamil2020agent}
models simulate a community where individuals represent ``agents'' in that community.
The pandemic course spreads among the agents based upon the virus assumptions and rules about social mixing, governmental policy and other behavioural patterns in the studied community.

\noindent \textbf{Curve-fitting}\cite{zhao2020well}
models refer to fitting a mathematical model by considering the current state and estimate the relationship between features of the pandemic.
The future of pandemic course can be approximated fully from assumptions about the contagion, public health policies or other limitations and uncertainties of spread disease parameters and/or experiences in other communities.

\noindent \textbf{Predictive}
models play a key role in the modern pandemic prediction.
Scientists apply different statistical and machine learning algorithms for modeling the future of morbidity and mortality of disease, and they produce state-of-the-art results even in the presence of many hidden variables.
Although powerful techniques sacrifice the interpretability to obtain accurate predictions, other post-hoc explainable techniques such as SHAP\cite{lundberg2017unified} or G-FORSE\cite{toutiaee2021gaussian} can be used for model interpretation. 
This approach is the core idea of this study which we discuss next.

The rest of this paper is organized as follows:
Section 2 focuses on the COVID-19 datasets and its different types of information collected by various sources, and their use cases in pandemic modeling while providing a focus on forecasting. 
Related work is reviewed in Section 3. 
Section 4 provides an overview of SEIR models with introducing common techniques for parameters estimation.
The predictive modeling techniques will be discussed extensively in Sections 5 and 6, starting from traditional statistical methods in Section 5, and the results are provided in Section 7.
Finally, conclusions and future work are given in Section 8.


==> tex/2-dataset.tex <==
This paper utilizes three datasets composed of data collected from multiple
datasets stored at
% \url{https://github.com/CSSEGISandData/COVID-19/tree/master/csse_covid_19_data}:
\url{https://covidtracking.com/data}
(1) Overall for the United States,
(2) State-by-State for the United States, and
(3) Covid-19 Government Response Tracker Data for the United States that includes Non-Pharmaceutical Interventions (NPI) at the state level.
% Average State Demographics, and Mobility Dataset (3) also includes data from LIST OTHER SOURCES.

\subsection{COVID-19 Dataset - United States}

The first {\sc ScalaTion} COVID-19 dataset
\url{https://github.com/scalation/data/COVID} contains data about COVID-19 cases, hospitalizations, recoveries, deaths and several more columns in the United States.
This dataset is in a CSV file with 367 rows and
18 columns containing the following data:

% \begin{table}[h]
% \label{tab:covid19_dataset1}
% \centering
% \caption{COVID-19 Dataset: United States}
% \begin{tabular}{|c|l|} \hline
% {\bf Column} & {\bf Description} \\ \hline \hline
% $d$          & date: January 22, 2020 to January 21, 2021 \\ \hline
% $t$          & time: 0 to 353 \\ \hline
% $C_t$        & total (cumulative) number of confirmed cases by day $t$ \\ \hline
% $H_t$        & total (cumulative) number of hospitalized individuals by day $t$ \\ \hline
% $R_t$        & total (cumulative) number of recovered individuals by day $t$ \\ \hline
% $D_t$        & total (cumulative) number of deaths by day $t$ \\ \hline \hline
% $I_t$        & deduced current number of infected individuals on day $t$ (not counting hospitalizations) \\ \hline
% $I_t^H$      & deduced current number of hospitalized individuals on day $t$ \\ \hline
% \end{tabular}
% \end{table}

\begin{table}[h]
\label{tab:covid19_dataset1}
\centering
\caption{COVID-19 Dataset: United States}
\begin{tabular}{|c|p{8.5cm}|}\hline
{\bf Column} & {\bf Description} \\ \hline
date          & date: January 19, 2020 to January 19, 2021 \\ \hline
death          & The cumulative number of deaths \\ \hline
deathIncrease        & The number of new deaths on the given date \\ \hline
inIcuCumulative       & The cumulative number of patients in ICU \\ \hline
inIcuCurrently       & The number of net total patients in ICU on the given date \\ \hline
hospitalizedIncrease        & The number of new hospitalizations on the given date \\ \hline 
%hospitalizedIncrease\_alt        & The number of new hospitalizations on the given date between 0.005 and 0.995 percentiles \\ \hline
hospitalizedCurrently     & The number of net total hospitalizations on the given date \\ \hline
hospitalizedCumulative     & The cumulative number of hospitalizations \\ \hline
negative     & The cumulative number of negative test results \\ \hline
negativeIncrease     & The number of new negative test results on the given date \\ \hline
onVentilatorCumulative     & The cumulative number of patients on ventilator \\ \hline
onVentilatorCurrently     & \scriptsize{The number of net total patients on ventilator on the given date} \\ \hline
positive     & The cumulative number of positive test results \\ \hline
positiveIncrease     & The number of new positive test results on the given date \\ \hline
states     & \scriptsize{The number of states reporting COVID-19 cases on the given date} \\ \hline
totalTestResults     & The cumulative number of total test results \\ \hline
totalTestResultsIncrease     & The number of total test results on the given date \\ \hline
recovered     & The cumulative number of recovered cases \\ \hline
\end{tabular}
\end{table}



\noindent
There are 367 rows in the dataset since the first row contains column headers
and the year 2020 was a leap year.

The data cover the last four states of the State Transition Diagram.
The data also include the total number of confirmed cases $C_t$
and the total number of hospitalizations $H_t$
that are not directly part of the $SEI^2RD$ model,
but are used to compute $I_t$ and $I_t^H$.
\begin{eqnarray*}
I_t   &=& C_t - H_t \\
I_t^H &=& H_t - R_t - D_t
\end{eqnarray*}

\subsection{COVID-19 Dataset - United States by State}

The second {\sc ScalaTion} COVID-19 dataset expands upon the previous one by splitting the data from the first one into counts for each state.
This dataset is in a CSV file with 18132 rows (first row is column headers) and 18 columns containing the same type of data.

\subsection{COVID-19 Dataset - U.S. Covid-19 Government Response Tracker}

The third {\sc ScalaTion} COVID-19 dataset provided in USNPI.CSV contains Covid-19 Government Response in the United States split by state that systematically collects information on several different common policy responses that government has taken to respond to the pandemic on 18 indicators such as business closures and travel restrictions.
Although this dataset stores mostly data about Non-Pharmaceutical Interventions (NPI) enforced by the administration, it also stores data about number of positive cases and deaths as well.


==> tex/3-related.tex <==
\subsection{Modeling Studies Reporting the Quality of the Forecasting}

Although there have been many paper that include forecasts for COVID-19,
only a fraction assess the quality of their forecasts.
The table below lists those that report that the Mean Absolute Percentage Error (MAPE) or a MAPE alternative measures.

The authors in \cite{kumar2020covid} forecasted the spread of disease in 10 mostly affected countries including the United States.
They applied ARIMA and Prophet time series forecasting models on the number of positive cases and deaths, and they showed that ARIMA outperformed FBProphet\cite{taylor2018forecasting} on scale of different error matrices such as MAPE and RMSE.
Another similar study that applied an ARIMA is found in \cite{ilie2020forecasting} where they extensively tested and tuned different parameters to minimize the prediction error, and they discussed that ARIMA models are appropriate for generating forecasts for the pandemic crisis.
Researchers in \cite{de2020long} evaluated two types of nonlinear regression models namely as Gompertz and Bertalanffy for the accumulated deaths of COVID-19 in six countries, and they concluded based on MAPE and the Relative Error (RE) criterion that Gompertz model was the one that best described the growth of deaths for some countries including the United States, and the Bertalanffy model was fitted well on China's data.
The predictive approach by machine learning was studied by \cite{prasanth2020forecasting} where they applied GWO-LSTM model to forecast the
the daily new cases, cumulative cases and deaths for India, USA and UK.
The network parameters of Long Short Term Memory (LSTM) network are optimized by Grey Wolf Optimizer (GWO), and they claimed that their hybrid architecture could obtained a better performance compared to the baseline (ARIMA).
Similarly, \cite{shastri2020time} proposed Stacked LSTM, Bi-directional LSTM and
Convolutional LSTM to forecast the COVID-19 cases for India and USA, and they concluded that the ConvLSTM performed better than the other two models for all four datasets of both countries.
And finally, \cite{tuli2020predicting} followed the curve fitting approach where they demonstrated that Generalized Inverse Weibull distribution showing a better fit than the baseline Gaussian model, and they discussed that using iterative weighting algorithm can improve the fitting performance.
\begin{small}
\begin{table}[h]
\begin{center}
\caption{Quality of COVID-19 Forecasting Models: {\bf C}ases and {\bf D}eaths}
\label{tab:textbooks}
\begin{tabular}{|l|l|c|c|c|c|c|c|} \hline
{\bf Paper} & {\bf Cite} & {\bf Variable} & {\bf Date} & {\bf Horizon} & {\bf Model} & {\bf Measure} & {\bf Quality} \\ \hline \hline
tuli2020predicting  & \cite{tuli2020predicting}  & $C$ & 5/4  & ?  & Gaussian     & MAPE & 1568.56 \\ \hline
tuli2020predicting  & \cite{tuli2020predicting}  & $C$ & 5/4  & ?  & Weibull      & MAPE & 26.58 \\ \hline \hline
shastri2020time     & \cite{shastri2020time}     & $C$ & 7/7  & 30 & S-LSTM       & MAPE & 10.00 \\ \hline
shastri2020time     & \cite{shastri2020time}     & $C$ & 7/7  & 30 & BD-LSTM      & MAPE & 6.66 \\ \hline
shastri2020time     & \cite{shastri2020time}     & $C$ & 7/7  & 30 & Conv-LSTM    & MAPE & 2.00 \\ \hline
shastri2020time     & \cite{shastri2020time}     & $D$ & 7/7  & 30 & S-LSTM       & MAPE & 8.00 \\ \hline
shastri2020time     & \cite{shastri2020time}     & $D$ & 7/7  & 30 & BD-LSTM      & MAPE & 6.00 \\ \hline
shastri2020time     & \cite{shastri2020time}     & $D$ & 7/7  & 30 & Conv-LSTM    & MAPE & 2.50 \\ \hline \hline
ilie2020forecasting & \cite{ilie2020forecasting} & $C$ & 7/10 & ?  & ARIMA(1,1,0) & MAPE & 3.22 \\ \hline \hline
de2020long          & \cite{de2020long}          & $D$ & 5/23 & 1  & Gompertz     & MAPE & 0.45 \\ \hline
de2020long          & \cite{de2020long}          & $D$ & 5/23 & 1  & Betalanffy   & MAPE & 6.82 \\ \hline \hline
prasanth2020forecasting & \cite{prasanth2020forecasting} & $C$ & 5/13 & 1 & ARIMA & MAPE & 10.36 \\ \hline
prasanth2020forecasting & \cite{prasanth2020forecasting} & $C$ & 5/13 & 1 & LSTM  & MAPE & 12.91 \\ \hline
prasanth2020forecasting & \cite{prasanth2020forecasting} & $D$ & 5/13 & 1 & ARIMA & MAPE & 9.52 \\ \hline
prasanth2020forecasting & \cite{prasanth2020forecasting} & $D$ & 5/13 & 1 & LSTM  & MAPE & 14.55 \\ \hline \hline
kumar2020covid      & \cite{kumar2020covid}      & $D$ & 5/20 & 1  & ARIMA(2,1,0) & MAPE & 2.57 \\ \hline
kumar2020covid      & \cite{kumar2020covid}      & $D$ & 5/20 & 1  & FBProphet    & MAPE & 5.75 \\ \hline
\end{tabular}
\end{center}
\end{table}
\end{small}
\subsection{The CDC Ensemble Model}
Every week, the Centers for Disease Control and Prevention (CDC) generates forecasts of COVID-19 cases and deaths over the next four weeks that ensemble the prediction from individual models submitted by different research groups.
Practically, it is observed that on the COVID-19 dataset, the improvements of ensemble technique over individual model forecasts are particularly pronounced.
This is in keeping with the previous work\cite{reich2019accuracy} in infectious disease forecasting and other fields that ensemble forecasts are often more accurate than any individual model going into the ensemble.
This work\cite{ray2020ensemble} described the performance of the ensemble forecast in more details.


==> tex/4-epidmodel.tex <==
The traditional SIR model proposed in Anderson (1991)\cite{anderson1991discussion} is a system of three ordinary differential equations that are non-linearly interrelated.
However, the extended version of this generative function has been proposed by successor researchers that has extra compartments in the equations, namely as $SEI^2R$, which we provide it in the following:



\begin{align*}
S_t &= S_{t-1} + d_t - e_t \\
E_t &= E_{t-1} + e_t - i_t \\
I_t &= I_{t-1} + i_t - i^H_t - r_t \\
I^H_t &= I^H_{t-1} + i^H_t - r_t - d_t \\
R_t &= R_{t-1} + r_t \\
D_t &= D_{t-1} + d_t 
\end{align*}

\begin{align*}
e_t &= a((I_t + I^H_t)*S_t/N) \\
i_t &= b(E_t) \\ 
i^H_t &= c(I_t) \\
r_t &= d_1I_t + d_2H_t \\
d_t &= e(I^H_t) 
\end{align*}

\begin{align*}
S_t &= N - (E_t + I_t + I^H_t + R_t)
\end{align*}


\begin{align*}
S_t   &= S_{t-1}   + \left[ q_5 I^H_{t-1} - \alpha \frac{I_{t-1} + I^H_{t-1}}{N} S_{t-1} \right] &&\text{Susceptible} \\
E_t   &= E_{t-1}   + \left[ \alpha \frac{I_{t-1} + I^H_{t-1}}{N} S_{t-1} - q_1 E_{t-1} \right]   &&\text{Exposed} \\
I_t   &= I_{t-1}   + \left[ q_1 E_{t-1} - (q_2 + q_3) I_{t-1} \right]   &&\text{only Infected} \\
I^H_t &= I^H_{t-1} + \left[ q_2 I_{t-1} - (q_4 + q_5) I^H_{t-1} \right] &&\text{Infected and Hospitalized} \\
R_t   &= R_{t-1}   + \left[ q_3 I_{t-1} + q_4 I^H_{t-1} \right]         &&\text{Recovered} \\
D_t   &= D_{t-1}   + \left[ q_5 I^H_{t-1} \right]                       &&\text{Died}
\end{align*}


% \begin{align*}
% S_t   &= S_{t-1}   + \Delta t \, \left[ q_5 I^H_{t-1} - \alpha \frac{I_{t-1} + I^H_{t-1}}{N} S_{t-1} \right] &&\text{Susceptible} \\
% E_t   &= E_{t-1}   + \Delta t \, \left[ \alpha \frac{I_{t-1} + I^H_{t-1}}{N} S_{t-1} - q_1 E_{t-1} \right]   &&\text{Exposed} \\
% I_t   &= I_{t-1}   + \Delta t \, \left[ q_1 E_{t-1} - (q_2 + q_3) I_{t-1} \right]   &&\text{only Infected} \\
% I^H_t &= I^H_{t-1} + \Delta t \, \left[ q_2 I_{t-1} - (q_4 + q_5) I^H_{t-1} \right] &&\text{Infected and Hospitalized} \\
% R_t   &= R_{t-1}   + \Delta t \, \left[ q_3 I_{t-1} + q_4 I^H_{t-1} \right]         &&\text{Recovered} \\
% D_t   &= D_{t-1}   + \Delta t \, \left[ q_5 I^H_{t-1} \right]                       &&\text{Died}
% \end{align*}

\noindent
See \cite{miller2020introduction} for a derivation of these difference equations. Several types of Kalman Filters \cite{sameni2020mathematical,li2017stochastic,arroyo2020tracking} are developed to study the dynamics of the COVID-19 Pandemic and make forecasts.

\begin{table}[h]
\label{tab:epidemiological_models}
\centering
\caption{Epidemiological Modeling Techniques}
\begin{tabular}{|c|l|} \hline
{\bf Modeling Technique} & {\bf Description} \\ \hline \hline
KF                       & Kalman Filter \\ \hline
EKF                      & Extended Kalman Filter \\ \hline
UKF                      & Unscented Kalman Filter \\ \hline
EnKF                     & Ensemble Kalman Filter \\ \hline
\end{tabular}
\end{table}

\subsection{Computing the Reproduction Number $R_0$}

==> tex/5-stat.tex <==
Several common statistical techniques for multi-variate time-series analysis may be applied to the COVID-19
datasets including the following.

\begin{table}[h]
\label{tab:statistical_models}
\centering
\caption{Statistical Modeling Techniques}
\begin{tabular}{|c|l|} \hline
{\bf Modeling Technique} & {\bf Description} \\ \hline \hline
$\text{RW}$             & Random Walk (Baseline) \\ \hline
$\text{SES}$            & Simple Exponential Smoothing \\ \hline
$\text{AR}(p)$          & Auto-Regressive of Order $p$ \\ \hline
$\text{ARIMA}(p, d, q)$ & Auto-Regressive, Integrated, Moving Average \\ \hline
$\text{SARIMA}$         & Seasonal ARIMA \\ \hline
Regression-TS            & Time-Series Regression \\ \hline
VAR                      & Vector Auto-Regressive  \\ \hline
VECM                     & Vector Error Correction Model \\ \hline
\end{tabular}
\end{table}

\subsection{Random Walk}
By definition, a candidate series follows a random walk if the first differences are random (non-stationary).
Random walk technique is commonly used in financial data analysis, and many studies have proved that many time series may be adequately modeled as a random walk, at least in the short term.
This model states the future value $y_t$ is the previous value $y_{t-1}$ disturbed by white noise $\epsilon_t$.

\begin{equation*}
y_t = y_{t-1} +\epsilon_t 
\end{equation*}
\noindent A stochastic process $\{\epsilon_t | t \in \{0,\ldots, m-1\}\}$ is considered to be white noise if:
\begin{align*}
\mathbb{E}[\epsilon_t] & = 0  &\text{zero mean}\\
\mathbb{E}[\epsilon_t^2] & = \sigma^2  &\text{constant variance}\\
\mathbb{E}[\epsilon_t\epsilon_{t-1}] & = 0  &\text{uncorrelated}
\end{align*}
\noindent Several distributions may be used to generate white noise with the most common being the Gaussian (Normal) distribution, $N(0,\sigma^2I)$.
Most packages in various data science toolkits perform a statistical significant test for stationarity/non-stationarity. 
The null hypothesis of the test is that the time series is non-stationary. 
So, it can be a candidate for random walk.

\subsection{Simple Exponential Smoothing}

\subsection{Auto-Regressive of Order $p$}
Another powerful technique for modeling time series data is the family of auto regressive. 
This method has been practiced for many years and it is popular among statisticians and economists.
The model equation for an AR$(p)$ model includes the past $p$ values.
Working with the zero-centered equations, we can derive a system of linear equations to solve for the parameters:
\begin{equation*}
z_t = \phi_0z_{t-p} + \phi_1z_{t-p+1} + \ldots + \phi_{p-1}z_{t-1} + \epsilon_t
\end{equation*}
\noindent Multiplying by $z_{t-k}$ and then taking the expectation produces:
\begin{equation*}
\gamma_k = \phi_0\gamma_{k-p} + \phi_1\gamma_{k-p+1} + \ldots + \phi_{p-1}\gamma_{k-1}
\end{equation*}
\noindent Dividing by $\gamma_0$ yields equations relating the parameters and correlations,
\begin{equation*}
\rho_k = \phi_0\rho_{k-p} + \phi_1\rho_{k-p+1} + \ldots + \phi_{p-1}\rho_{k-1}    
\end{equation*}
\noindent These equations contain $p$ unknowns and by letting $k = 1,2,\ldots,p$, it can be used to generate $p$ equations, or one matrix equation.

\subsection{Auto-Regressive Integrated Moving Average}
The ARMA class provides basic time-series analysis capabilities for Auto-Regressive (AR) and Moving Average (MA) models.
In an ARMA$(p,q)$ model, $p$ and $q$ refer to the order of the Auto-Regressive and Moving Average components of the model, respectively.
In cases where a time-series is not stationary, an ARIMA$(p,d,q)$ may be used.
The new hyper-parameter $d$ is the number of times the time-series is differenced. 
When there is a trend in the data (e.g., the values or levels are increasing over time), an ARIMA$(p, 1, q)$ may be effective. 
This model will take a first difference of the values in the time-series, namely as:
\begin{equation*}
y'_t = y_t - y_{t-1}
\end{equation*}

\subsection{Seasonal ARIMA}
The word ``seasonal'' is used to mean any time period longer than one. 
Seasonal ARIMA allows for seasonal differences, so a SARIMA$(p,d,q)\times(0,D,0)_s$ is:
\begin{equation*}
\phi.[-B^p,\ldots,-B^1,1](1-B)^d(1-B^s)^Dy_t = \delta + \bm{\theta}.[B^q,\ldots,B^1,1]\epsilon_t
\end{equation*}
\noindent The seasonal differencing $(1-B^s)^D$ happens first, followed by regular differencing $(1-B)^d$ and then essentially an an ARMA model.
In addition, seasonal autoregressive parameter vector $\phi^s \in \mathbb{R}^p$ and seasonal moving-average parameter vector $\bm{\theta}^s \in \mathbb{R}^Q$ may be added to a SARIMA$(p,d,q)\times(P,D,Q)_s$ model:
\begin{eqnarray*}
[\phi.[-B^p,\ldots,-B^1,1]][\phi^s.[-B^{sp},\ldots,-B^s,1]](1-B)^d(1-B^s)^D y_t = \\
\delta + [\bm{\theta}.[B^q,\ldots,B^1,1]][\bm{\theta}^s.[B^{sq},\ldots,B^s,1]]\epsilon_t
\end{eqnarray*}
\noindent The expression $[\phi.[-B^p,\ldots,-B^1,1]]$ may be viewed as a polynomial and the polynomials are multiplied, therefore, it is referred to as a multiplicative SARIMA model.

\subsection{Time-Series Regression}
One of the simplest forms of forecasting in time-series is regression with lagged variables.
Given a predictor time-series $\{x_t\}$ and a response time-series $\{y_t\}$, a simple time-series regression model uses the current value of $x_t$ to predict $y_t$.
\begin{equation*}
y_t = b_0 + b_1x_t + \epsilon_t
\end{equation*}
\noindent Knowing previous values of $x_t$ often helps with the predictions, so it is common to introduce a lagged predictor variable $x_{t-1}$.
One may also introduce a lagged response variable $y_{t-1}$
\begin{equation*}
y_t = b_0 + \phi_1y_{t-1} + b_1x_t + b_2x_{t-1} + \epsilon_t
\end{equation*}
\noindent The expression above may introduce estimation problems for Ordinary Least Squares (OLS) or Generalized Least Squares (GLS) which both have been practiced in many domains.
While $x_t$ may be dropped from the model equation if contemporaneous values are not known, these equations can be extended to multiple predictor variables and multiple lags.

\subsection{Vector Auto-Regressive}
If multiple variables involve in forecasting, Multivariate Time-Series Analysis (MTSA) may be used.
MTSA extends univariate time-series by analyzing multiple variables. 
It works on multiple interrelated time-series,
\begin{equation*}
\mathbf{y}_t = \{y_{t0},y_{t1},\ldots, y_{t,n-1}\}
\end{equation*}
\noindent with one time-series for each of the $n$ variables.
The forecasted value for the $j^{th}$ variable at time t, $y_{tj}$, can depend on the previous (or lagged) values of all the variables.
This notion is captured in Vector Auto-Regressive models \cite{zivot2006vector}.
A vector auto-regressive model of order $p$ with $n$ variables, VAR$(p,n)$, will utilize the most recent $p$ values for each variable to produce a forecast.
The equation for the response vector $\mathbf{y}_t \in \mathbb{R}^n$ may be written in matrix-vector form as follows:
\begin{equation*}
\mathbf{y}_t = \delta +\Phi^{(0)}\mathbf{y}_{t-p} + \Phi^{(1)}\mathbf{y}_{t-p+1} + \ldots + \Phi^{(p-1)}\mathbf{y}_{t-1} + \epsilon_t
\end{equation*}
\noindent where constant vector $\bm{\delta} \in \mathbb{R}^n$, parameter matrices $\Phi^{(l)} \in \mathbb{R}^{n\times n} (l = 0, \ldots, p - 1)$, and error vector $\epsilon_t \in \mathbb{R}^n$.

\subsection{Vector Error Correction Model}



==> tex/6-ml.tex <==
Although there are many type of machine learning techniques that could be applied,
this paper focuses on various types of Neural Networks and Deep Learning.

\begin{table}[h]
\label{tab:machine_learning_models}
\centering
\caption{Machine Learning Techniques}
\begin{tabular}{|c|l|} \hline
{\bf Modeling Technique} & {\bf Description} \\ \hline \hline
Neural Network-TS        & Neural Network for Time-Series \textcolor{blue}{IJ}\\ \hline
GRU                      & Gate Recurrent Unit \textcolor{blue}{IJ}\\ \hline
LSTM                     & Long, Short-Term Memory \textcolor{blue}{IJ}\\ \hline
Conv-LSTM                & Convolutional-LSTM \textcolor{blue}{IS - IJ}\\ \hline
EncoderDecoder-LSTM      & Encoder-Decoder-Attention-LSTM \textcolor{blue}{YC}\\ \hline
GNN-LSTM                 & Graph Neural Network-LSTM \textcolor{blue}{RM}\\ \hline
Transformer-LSTM         & Transform-LSTM \textcolor{blue}{MA}\\ \hline
Hybrid                   & Complementary Composition of Models \textcolor{blue}{??}\\ \hline
\end{tabular}
\end{table}

\subsection{Neural Network for Time-Series}
With the extension of Neural Network models in many application, we can forecast time-series data with such sophisticated methods.
an Auto-Regressive Neural Network ARNN$(p)$ model is a special case of a $p^{th}$ order Nonlinear Auto-Regressive NAR$(p)$ model, which is a generalization of an $AR(p)$ model.
It is a three-layer (one hidden) neural network, where the input layer has a node for each of the $p$ lags, the hidden layer also has $p$ nodes, and the output layer has 1 node:
\begin{eqnarray*}
\mathbf{x}_t & = & [y_{t-p},\ldots,y_{t-1}]\\
y_t &=& \mathbf{w}.\mathbf{f(\Phi x_t)} + \epsilon_t
\end{eqnarray*}
\noindent the $p\times p$ matrix $\Phi$ holds the parameters/weights connecting the input and hidden layers, while the $p$ dimensional vector $\mathbf{w}$ holds the parameters/weights connecting the hidden and output layers.
There is only an activation function (vectorized $\mathbf{f}$) for the hidden layer.

\subsection{Long Short-Term Memory}
Long Short-Term Memory (LSTM) \cite{hochreiter1997long} has been proposed many years ago to fix some issues that a simple Recurrent Neural Network model may face during the training process, and many experiments have proved that this particular method is actually effective.

\subsection{Gate Recurrent Unit}
In recent years, some group of researchers have improved the LSTM model by simplifying its architecture, and they introduced Gated Recurrent Unit (GRU) which became popular among the researchers.
It adds a second gate, a third parameter matrix and a third bias vector.
The two gates in a GRU are the \textit{reset gate} and the \textit{update gate}.
The equations below show how information flows through a gated recurrent unit \cite{cho2014learning,yu2019review,zhou2016minimal}:
\begin{align*}
\mathbf{x_t} & = [y_{t-1},\ldots,y_{t-p}] & \text{input} \\
\mathbf{r_t} & = f_1(\Psi [\mathbf{h_{t-1}},\mathbf{x_t}]+\beta_r) & \text{reset gate} \\
\mathbf{u_t} & = f_2(\Phi [\mathbf{h_{t-1}},\mathbf{x_t}]+\beta_u) & \text{update gate} \\
\mathbf{\Tilde{h}_t} & = f_3(\Theta [r_t\odot \mathbf{h_{t-1}},\mathbf{x_t}]+\beta_h) & \text{candidate state} \\
\mathbf{h_t} & = (\mathbf{1}-\mathbf{u_t}) \odot \mathbf{h_{t-1}} + \mathbf{u_t} \odot\mathbf{\Tilde{h}_t} & \text{state} \\
y_t & = \mathbf{h_t}(0) + \epsilon_t &\text{output}
\end{align*}
\noindent The parameters consist of three weight/parameter matrices $\bm{\Phi} \in \mathbb{R}^{p\times 2p}$, $\bm{\Psi} \in \mathbb{R}^{p\times 2p}$ and $\bm{\Theta} \in \mathbb{R}^{p\times 2p}$, as well as three bias vectors $\beta_z \in \mathbb{R}^p$, $\beta_r \in \mathbb{R}^p$ and $\beta_h \in \mathbb{R}^p$.
The first two activation functions default to \textit{sigmoid}, while the third activation function defaults to \textit{tanh}.

The vanishing gradient issue in GRU is managed by an update gate and a reset gate. 
The update gate and reset gate control information that flows into and out of memory, respectively.

\subsection{Convolutional-LSTM}

The Convolutional LSTM or ConvLSTM \cite{shi2015convolutional} is constructed upon the fully connected LSTM (FC\_LSTM), where it extends the idea of having convolutional structures in both the input-to-state and state-to-state transitions.
In comparison with other simple RNN network architectures, such as LSTM or GRU, this combined architecture encourages the process to determine the future state of a certain cell in the grid by the inputs and past states of its local neighbors.
By stacking multiple ConvLSTM layers and forming an encoding-forecasting structure, it is possible to build an end-to-end trainable model for spatio-temporal casting. 
Like other RNN models, it has feedback connections, making it useful to process entire sequences of data. 
The ConvLSTM is formulated as follow:
\begin{eqnarray*}
i_t &=& \sigma (W_{xi}X_t + W_{hi}H_{t-1} + W_{ci}\odot C_{t-1} + b_i) \\
f_t &=& \sigma (W_{xf}X_t + W_{hf}H_{t-1} + W_{cf}\odot C_{t-1} + b_f) \\
C_t &=& f_t \odot C_{t-1} + i_t \odot tanh (W_{xc}X_t + W_{hc}H_{t-1}+b_c) \\
o_t &=& \sigma (W_{xo}X_t + W_{ho}H_{t-1} + W_{co}\odot C_{t} + b_o) \\
H_t &=& o_t \odot tanh(C_t)
\end{eqnarray*}

\subsection{Encoder-Decoder-Attention-LSTM}
The encoder–decoder model uses an LSTM based encoder that learns vector representations from input time series. 
These encoded representations have to be of a fixed length. 
This representation is then fed into an LSTM based decoder whose job is to reconstruct the time series using the current hidden state and the output of the previous time step \cite{malhotra2016lstm}. 
Since the encoded representations have to be of a fixed length, capturing all the information from input series can be challenging \cite{bahdanau2014neural}. 
It is also difficult to capture long term dependencies since previous memories are erased and the model is refreshed with new observations \cite{fan2019multi}. 
To combat this problem, attention mechanisms can be incorporated in the decoder. 
An alignment score is generated for each time step of the encoder and the decoder uses a weighted sum. 
The alignment scores are then normalized using softmax function to obtain attention weights. 
A context vector is then built as the weighted sum of hidden values of the encoder and the attention weights. 
This context vector is used to compute the current hidden state of the decoder using the hidden state of the previous step and the output of the previous step. 
Once the hidden state is computed for each time step, the output of the decoder can be computed using softmax on weighted hidden state \cite{gangopadhyay2018temporal}.

\subsection{Graph Neural Network-LSTM}
one of the interesting topics in network science and knowledge graph is Graph Neural Network (GNN) models, which is gradually receiving tons of attentions by practitioners.
A Graph Convolutional Network (GCN) is a special case of GNN, where it takes the advantage of convolutional layers for aggregating the neighbors' information at each node.
In GCN models the entities or nodes are connected by some edges, where those edges can represent distance, correlation and causality \cite{przymus2017improving}.
The GCN\_LSTM captures the spatial dependency of the underlying graph network by the GCN component, and the dynamic dependency of the graph is captured by the LSTM, together forming a hybrid architecture that takes the advantage of combining two complex deep frameworks.

\subsection{Transformers}
In addition to using popular recurrent neural networks to model our sequential data, we attempt to use other class of transduction models which are transformer models. Transformer models have been successful on modeling sequential data, such as language data, by achieving state of the art results on machine translations \cite{vaswani2017attention}. The transformer models replace the recurrent and the convolutional neural networks by solely relying on multiheaded self-attentions to capture the temporal and complex global dependencies \cite{vaswani2017attention}. Such models also allow for parallelization which is ideal for modeling long sequences \cite{vaswani2017attention}. The architecture of the transformer models consists of stacked encoders and decoders. The encoder consists of positional embedding, multiheaded self-attentions, and a feed-forward layer \cite{wu2020deep}. The decoder consists of positional encoding, multiheaded attention applied to the encoded sequence, masked multiheaded attention applied to the output sequence, and a feed-forward layer \cite{wu2020deep}. The transformer models have gained attention recently to model time series data, such as forecasting seasonal influenza epidemics.   

\subsection{Complementary Composition of Models}

==> tex/7-res.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% de
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!ht]
    \centering
    \caption{sMAPE values for different models.}
        \begin{tabular}{c c c c c c c}
            \toprule
            \midrule
                & & \multicolumn{5}{c}{sMAPE Values}\\ \cmidrule{3-7}
                && Deaths  & Cases & Hospitalizations &  &\\ \cmidrule{3-7}
                \multicolumn{1}{c}{\multirow{15}{*}{\begin{sideways}\parbox{2cm}{\centering Models}\end{sideways}}}  &
                \multicolumn{1}{r}{RW}& 30.98 & ? & ? &  \\
                \multicolumn{1}{c}{}    &
                \multicolumn{1}{r}{SES}& ? & ? & ? &\\
                \multicolumn{1}{c}{}    &
                \multicolumn{1}{r}{AR(p)} & 39.04 & ? & ? &\\
                \multicolumn{1}{c}{}    &   
                \multicolumn{1}{r}{ARIMA(p,d,q)} & 20.46 & ? & ? & \\
                \multicolumn{1}{c}{}    &
                \multicolumn{1}{r}{SARIMA} & 19.30 & ? & ? &\\
                \multicolumn{1}{c}{}    &
                \multicolumn{1}{r}{Regression-TS} & 42.27 & ? & ? &  \\
                \multicolumn{1}{c}{}    &
                \multicolumn{1}{r}{QuadRegression-TS} & 42.05 & ? & ? &  \\
                \multicolumn{1}{c}{}    &
                \multicolumn{1}{r}{QuadXRegression-TS} & 38.85 & ? & ? &  \\
                \multicolumn{1}{c}{}    &
                \multicolumn{1}{r}{VAR} & ? & ? & ? &\\
                \multicolumn{1}{c}{}    &
                \multicolumn{1}{r}{VECM} & ? & ? & ? & \\
                \multicolumn{1}{c}{}    &   
                \multicolumn{1}{r}{Neural Network-TS} & 26.10 & ? & ? & \\
                \multicolumn{1}{c}{}    &
                \multicolumn{1}{r}{GRU} & ? & ? & ? &\\
                \multicolumn{1}{c}{}    &
                \multicolumn{1}{r}{LSTM} & ? & ? & ? & \\
                \multicolumn{1}{c}{}    &
                \multicolumn{1}{r}{Conv-LSTM} & ? & ? & ? &\\
                \multicolumn{1}{c}{}    &
                \multicolumn{1}{r}{EncoderDecoder-LSTM} & ? & ? & ? & \\
                \multicolumn{1}{c}{}    &   
                \multicolumn{1}{r}{GNN-LSTM} & ? & ? & ? & \\
                \multicolumn{1}{c}{}    &
                \multicolumn{1}{r}{Transformer-LSTM} & ? & ? & ? &\\
            \midrule
            \bottomrule
        \end{tabular}
        \centering
        \label{tab:de}
\end{table*}


\begin{small}
\begin{table}[!h]
\begin{center}
\caption{Multi-Horizon ($h$) Rolling Forecasts: Baseline and Other Models (sMAPE).}
\label{tab:}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} \hline
Horizon   & Random Walk & ARIMA(p, 0, 0)  & ARIMA(p, 0, 1) & SARIMA(p, 0, 1)(3, 1, 3)\\ \hline \hline
in-sample & 29.31  & 21.85 (9)   & 21.80 (8)  & 16.75 (6)  \\ \hline
$h = 1$   & 31.63  & 14.80 (10)  & 27.50 (3)  & 13.60 (1)  \\ \hline
$h = 2$   & 52.78  & 16.50 (10)  & 35.00 (6)  & 15.70 (1)  \\ \hline
$h = 3$   & 56.80  & 16.40 (10)  & 33.90 (5)  & 15.80 (2)  \\ \hline
$h = 4$   & 56.45  & 16.70 (9)   & 33.70 (8)  & 16.30 (4)  \\ \hline
$h = 5$   & 52.24  & 17.20 (9)   & 33.20 (8)  & 16.80 (4)  \\ \hline
$h = 6$   & 33.08  & 17.40 (8)   & 31.90 (8)  & 16.90 (4)  \\ \hline
$h = 7$   & 16.90  & 17.30 (9)   & 31.40 (8)  & 16.90 (6)  \\ \hline
$h = 8$   & 33.42  & 20.80 (9)   & 33.90 (8)  & 19.00 (4)  \\ \hline
$h = 9$   & 50.72  & 22.30 (9)   & 36.40 (8)  & 20.30 (4)  \\ \hline
$h = 10$  & 54.80  & 22.10 (9)   & 35.70 (8)  & 20.40 (6)  \\ \hline
$h = 11$  & 55.58  & 22.20 (9)   & 36.70 (8)  & 20.40 (4)  \\ \hline
$h = 12$  & 51.29  & 23.10 (9)   & 37.90 (8)  & 21.70 (4)  \\ \hline
$h = 13$  & 33.95  & 23.00 (9)   & 36.90 (3)  & 21.80 (4)  \\ \hline
$h = 14$  & 22.32  & 23.10 (9)   & 37.00 (8)  & 21.60 (7)  \\ \hline
\end{tabular}
\end{center}
\end{table}
\end{small}















